Non-Intrusive Adaptation: Input-Centric Parameter-efficient Fine-Tuning for Versatile Multimodal Modeling

Large language models (LLMs) and vision language models (VLMs) demonstrate excellent performance on a wide range of tasks by scaling up parameter counts from O(10^9) to O(10^{12}) levels and further beyond. These large scales make it impossible to adapt and deploy fully specialized models given a task of interest. Parameter-efficient fine-tuning (PEFT) emerges as a promising direction to tackle the adaptation and serving challenges for such large models. We categorize PEFT techniques into two types: intrusive and non-intrusive. Intrusive PEFT techniques directly change a model's internal architecture. Though more flexible, they introduce significant complexities for training and serving. Non-intrusive PEFT techniques leave the internal architecture unchanged and only adapt model-external parameters, such as embeddings for input. In this work, we describe AdaLink as a non-intrusive PEFT technique that achieves competitive performance compared to SoTA intrusive PEFT (LoRA) and full model fine-tuning (FT) on various tasks. We evaluate using both text-only and multimodal tasks, with experiments that account for both parameter-count scaling and training regime (with and without instruction tuning).

==> subfiles/4_exp_backup.tex <==
\section{Experiments}
% \input{subfiles/_pali_results}


\subsection{Multimodal Experiments}
% checkpoint details: IT
% MMIT
We conduct PEFT experiments on four VQA and two image captioning tasks using PaLI models \citep{chen2023pali}, a family of multi-modal foundational models that have achieved SoTA results on a wide range of vision and language benchmarks. We demonstrate that non-intrusive PEFT achieve very competitive results compared to full model fine-tuning for base models with higher parameter counts and instruction tuned.


\subsubsection{Base Models}
We consider four variants of PaLI models: base models at two different sizes, and whether pretraining included a multimodal instruction tuning (MMIT) stage at each size.

\textbf{PaLI models:} for the large-scale model, we consider PaLI-X \citep{chen2023pali} with 55B parameters; we use the checkpoint pre-trained per \citet{chen2023pali} with a resolution of 756 $\times$ 756.  We also consider a (relatively) small-scale model, a 5B variant of PaLI, pre-trained with similar objectives at a higher resolution (812 $\times$ 812) and better text understanding capabilities.

\textbf{MMIT:} Due to the limitation and digression of the task scopes in most public academic benchmarks, we create the MMIT task collections in the spirit of ``Self-Instruct'' \citep{wang2022self}, taking advantages of the powerful large language models. We consider 3 clusters of tasks: (i) Long-form captioning where LLMs \citep{anil2023palm} are used to combine and summarize different generated captions for each image; (ii) Creative writing where LLMs are used to generate both the novel creative writing prompts and the actual writings given the prompts based on image captions. (iii) Long-form question answering where LLMs are used to generate the both questions and answers accompanied with rationales given image captions. Although we only have 3 cluster of tasks, each cluster covers closer and comprehensive aspects to natural daily use cases. We finetune the pre-trained raw PaLI models on the MMIT collections for 17k steps to produce the MMIT checkpoints. We note the generated tasks covered in the MMIT are comprehensive yet general, we do not expect them to do directly relevant to specific down-stream tasks. In particular, we experiment on down-stream tasks that require specific skills such as understanding scene texts and documents and answering knowledge intensive questions.

\subsubsection{Implementation Details}
Fine tuning and three types of PEFT including prompt tuning \citep{prompt_tuning}, LoRA \citep{hu2021lora} and \sysname  are examined in this work. We employ adafactor \citep{shazeer2018adafactor} as the optimizer. The learning rate is set to 0.03 for the PEFT and 0.0001 for fine tuning with a linear warmup and reciprocal square root decay  if not otherwise specified. We set the dropout rate as 0.1 to prevent over-fitting. 

\textbf{LoRA.} We add LoRA weights on each linear layer in the multi-head attention and the MLP blocks in the encoder transformer blocks for all the PaLI models. Similar to \citep{yang2022prompt}, we found that adding LoRA weights in the decoder does not help the adaptation performance much at while costing twice as much as parameter counts. We use a LoRA rank of 16 in all the experiments except for the PaLI-X MMIT experiments that use a rank of 4.

\textbf{Prompt Tuning.} PT is implemented on the input to the multimodal Encoder-Decoder in PaLI, concatenating $64$ soft tunable tokens to the embeddings of the text tokens and the visual tokens from the frozen ViT. We apply two layers of residual re-parameterization \citep{razdaibiedina2023residual} for more stable results. We use a dropout rate of 0.05 for all prompt tuning experiments as we found it outperforming the default rate of 0.1

\textbf{AdaPrompt}. We insert the \sysname to the embeddings of the text tokens and the visual tokens from the frozen ViT as a non-intrusive PEFT to the PaLI's Encoder-Decoder. We use a rank of $64$ in all the experiments.



\subsubsection{Image captioning Results}

\begin{table}[h]
\scriptsize
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{1}{c|}{}         & \multicolumn{6}{c|}{PaLI-5B}                                                       & \multicolumn{6}{c}{PaLI-55B}                                                      \\ \hline
& \multicolumn{2}{c}{COCO} & \multicolumn{2}{c}{Textcaps} & \multicolumn{2}{c|}{avg. $\delta$ to FT} & \multicolumn{2}{c}{COCO} & \multicolumn{2}{c}{Textcaps} & \multicolumn{2}{c}{avg. $\delta$ to FT} \\
             & raw         & MMIT       & raw           & MMIT         & raw         & MMIT      & RAW         & MMIT       & RAW           & MMIT         & raw        & MMIT   \\\hline
FT            & 145.9       & 144.7      & 158.8         & 160.1        & 0           & 0         & 147.4       & 147        & 148.6         & 148.5        & 0          & 0        \\ 
LoRA          & 145.5       & 145.7      & 160.4         & 159.5        & +0.6        & +0.2       & 146.1       & 146.8      & 147.8         & 148.6        & -1.05      & -0.05    \\ \hline
Prompt-tuning            & 140.2       & 140.9      & 155           & 155.5        & -4.75       & -4.2      & 143.5       & 142.2      & 144.9         & 145.5        & -3.8       & -3.9     \\
\sysname      & 142.9       & 144.6      & 158.7         & 158.6        & -1.55       & -0.8      & 146.2       & 146.3      & 145.2         & 147.9        & -2.3       & -0.65    \\
\bottomrule
\end{tabular}
\caption{PEFT results on COCO and textcaps captioning tasks on the validation splits. We report cider score for each task. \sysname consistently outperforms prompt tuning as non-intrusive PEFT approaches and achieves competitive results to FT.}
\label{tab:mm_cap_results}
\end{table}

We report the PEFT image captioning cider scores \citep{vedantam2015cider} on COCO \citep{lin2014microsoft} and TextCaps \citep{sidorov2020textcaps} using the validation splits in table \ref{tab:mm_cap_results}. Within the non-intrusive PEFT family, \sysname outperforms prompt tuning by about 3 cider points on PaLI-5B and 2 cider points on the PaLI-X model, indicating the effectiveness of directly adapting the input embeddings. 

We observe smaller gaps between \sysname and FT on MMIT than the raw checkpoints for both PaLI-5B and PaLI-X models, supporting our hypothesis that PEFT approaches are able to benefit more from scaling up the pre-training tasks and demonstrate competitive results to FT. Practically speaking, as the instruction tuned LLM checkpoints occupied increasingly more market of the use case, non-intrusive PEFT, especially \sysname, become a strong candidate that significantly reduces the complexities in architecture and serving infrastructure at a cost of very minor performance degradation. As the model sizes keep growing larger and the instruction tuning tasks being more comprehensive, we expect to see even closer performance between simple non-intrusive PEFT approach like \sysname and intrusive PEFT or FT. As the non-intrusive PEFT approaches does not scale along with the depth of the growing models, they present clear advantages in terms of practicality.


\textbf{Effect of the rank.} Table \ref{tab:rank_COCO} reports the effects of changing the ranks in \sysname on COCO karparthy test set using PaLI MMIT checkpoints of both sizes. We observe that the performances are not very sensitive to the rank, indicating the stability of the \sysname. Even a rank of 4 can help the models adapt to reasonable performances and the performance saturated at a rank of 64 for the both models.


\begin{table}[h]
\centering
\begin{tabular}{l|cccc|l|cccc}
\toprule
        &  4   & 16   &  64   & 256    &        &  4  & 16   & 64   & 256   \\ \hline
PaLI-5B & 141.0   & 143.4   &  144.6   & 144.8    & PaLI-X &  144.5 & 145.3   & 146.3   & 146.3   \\ \bottomrule  
   
\end{tabular}
\caption{Effect of rank in \sysname on the COCO captioning task. }
\label{tab:rank_COCO}
\end{table}


\subsubsection{VQA Results}
In table \ref{tab:mm_vqa_results}, we present VQA performances using PEFT on four VQA tasks, covering outside knowledge VQA (OK-VQA) \citep{marino2019ok}, document understanding VQA (DocVQA) \citep{mathew2021docvqa}, and two scene-text understanding datasets, i.e. TextVQA \citep{singh2019towards} and ST-VQA \citep{biten2019scene}. We follow standard evaluation metrics, using soft accuracy \citep{antol2015vqa} for OKVQA and TextVQA and ANLS score for DocVQA and ST-VQA.


\begin{table}[h]
\scriptsize
\begin{tabular}{lc|c|cccccccccc}
\toprule
Tuning  &Non-intru- & \#params & \multicolumn{2}{c}{OKVQA} & \multicolumn{2}{c}{DocVQA} & \multicolumn{2}{c}{ST-VQA} & \multicolumn{2}{c}{TextVQA} & \multicolumn{2}{c}{avg. $\delta$ to FT}  \\
Approach   & sive &          & Raw        & MMIT         & Raw        & MMIT          & Raw          & MMIT        & Raw        & MMiT           & RAW         & MMIT            \\\midrule
FT & No & 3B$^\dag$      & 60.1       & 61.13        & 83.3       & 81.3          & 83.6         & 83.1        & 76.5       & 75.4           & 0           & 0              \\
LoRA  & No &          & 57.34      & 58.33        & 83         & 82.1          & 82.2         & 83          & 76.3       & 76.4           & -1.17       & -0.28          \\
Prompt-tuning &Yes & 131k     & 57.55      & 59.1         & 80.3       & 79.66         & 82.6         & 82.2        & 76.1       & 76.3           & -1.74      & -0.92         \\
\sysname   &Yes  & 524k     & 56.8       &  56.7    & 78.3         & 78.6      & 81.6         & 81.9        & 75.4       &   74.7     &    -2.93   & -2.33    \\\midrule
FT  & No& 32B$^\dag$       & 66.1        & 66.9        & 80.0         & 82.8        & 80.2         & 79.7        & 71.9         & 70.7         & 0.0           & 0.0       \\     
LoRA        & No& 19M    & 63.3        & 67.1        & 80.6         & 83.2        & 78.6         & 80.0        & 69.1         & 70.8         & -1.7          & +0.25         \\
Prompt tuning  &Yes& 262k     & 64.9        & 66.4        & 79.7         & 82.4        & 78.3         & 79.8        & 69.7         & 70.4         & -1.4          & -0.3           \\
\sysname     &Yes & 1.05M    & 63.9        & 66.8        &    78.3     & 82.9        & 77.9         & 80.0        &      67.8        & 70.2         &     -2.58          & -0.05          \\ \bottomrule

\end{tabular}
\caption{PEFT results on four VQA tasks on the validation splits. The first and second half present the results on the PaLI-5B and the PaLI-X models, respectively. $^\dag$ We only fine tune the Encoder-Decoder part of the PaLI model and leave the ViT part frozen. }
\label{tab:mm_vqa_results}
\end{table}


For the PaLI-5B raw model, LoRA as an intrusive PEFT approach achieves the most competitive average results to the FT results, yielding only 1.17 performance degradation where both prompt tuning and \sysname achieve worse results, yielding 1.74 and 2.93 performance degradation. We attribute this to the strong expression capabilities offered by the flexibility in modifying the internal architecture. Within non-intrusive PEFT, \sysname falls behind prompt tuning by 1.2 points. We hypothesize that the adapters in \sysname from different modalities learn to separately over fit modality bias rather than collaborating to learn to reason the visual questions given the image. 

Both issues are addressed with the help of scaling up both the parameter counts and the pre-training tasks. On the PaLI-55B MMIT model, the average performance differences on the MMIT checkpoint are negligible that only lose a score of 0.05 to FT, highlighting that \sysname emerges to be an excellent choice considering the ease of serving and the parameter counts. 

It is worth noting that all three PEFT approaches, including both intrusive and non-intrusive variants, present better performances with scaling up both parameter counts and tasks, achieving competitive performances to FT. This reveals and supports the trend towards PEFT where the LLMs and VLMs are increasingly powerful and only little adaptation is needed to achieve optimized performance for specialized use cases, relieving the need of directly learning the domain knowledge. Comparing to intrusive PEFT that are more similar to FT in spirits of adapting internal parameters, non-intrusive PEFT approaches like \sysname are often sufficient and offer similar performances with significant ease of model deployment and constant parameter counts with respect to the model depth. 


% 1. Main performance table
% @yaqingwang
% Raw T5: GLUE Tydiaqa QA
% FLAN 

% QA: HotpotQA (Yang et al., 2018), NewsQA (Trischler
% et al., 2017) and SearchQA (Dunn et al., 2017) from MRQA (Fisch et al., 2019); WinoGrande (Sakaguchi et al., 2021), Yelp-2 (Zhang et al., 2015), SciTail (Khot et al., 2018) and PAWS-Wiki



% @jialinwu
% Raw
% MMIT
% Dataset: COCO, textcaps, VATEX, VQA-v2, OKVQA, ST-VQA, NextQA






% 1. Good performance
% 2. IT reduce parameter needed



% 2. Baseline
% lora, prompt tuning, adaprompt 

% 1. Text: T5 xxl + LoRA ? @yaqingwang
% 2. Multimodal LoRA: READY 


% lora, prompt tuning--GLUE

% 3. Difficult to optimize @yaqingwang
% Multi-task for prompt tuning, adaprompt
% Small checkpoint with T5 large to show better peformance
% https://openreview.net/pdf?id=Nk2pDtuhTq


% 4. Serving cost/inference speed:
% 1. LoRA v.s. Adaprompt 
% @jialin

% 5. Few-shot (16 shots, 32 shots, 128 shots) in IT models
% i. multimodal @jialin
% ii. text @yaqingwang




% 6. adaprompt multimodal albation 


% 7 server inference speed 

\subsection{Natural Language Experiments}

\noindent\textbf{Experimental setting.} We perform experiments on a wide range of tasks including eight natural language understanding (NLU) tasks in the General Language Understanding Evaluation (GLUE) benchmark \cite{wang2019glue}. We compare
{\sysname} to full model fine-tuning with various checkpoints including instruction-tuned checkpoint FLAN~\citep{wei2021finetuned} and T5 checkpoints with additional adaption steps following ~\citep{prompt_tuning}. Unless otherwise specified, all of the experiments in this work utilize the 11 billion parameter T5 checkpoint as the base model.

\noindent{\bf AdaPrompt implementation details.} We implement {\sysname} in Jax for experiments. {\sysname} uses a dimension $r$ of $4$ and $256$ with FLAN and T5 checkpoint in single task setting. In multi-task setting, we increase the dimensions to $256$ and $1024$ for FLAN and T5 checkpoints respectively. We found that most of tasks are not sensitive to rank of {\sysname} and  the performance of {\sysname} plateaus after the modules reach a certain size. Increasing the capacity beyond this point yields diminishing returns, with little to no improvement observed in the end task metrics.



\noindent\textbf{Single task.} The table compares full fine-tuning versus using {\sysname} for adapting T5-11B to individual GLUE tasks. For full fine-tuning, all 11 billion parameters are tuned on each task. With {\sysname}, only the small adapter modules with 0.5-0.008 million parameters are tuned per task. We observe that {\sysname} achieves comparable or better performance than full fine-tuning on most tasks, despite tuning far fewer parameters. For example, with the FLAN checkpoint, {\sysname} attains higher accuracy on SST-2, QQP, RTE and STS-B benchmarks. Overall, {\sysname} achieves a similar average GLUE score to full fine-tuning of 90.7 using FLAN, while only tuning 0.008M adaption parameters per task. This demonstrates {\sysname}'s effectiveness in targeted task adaptation for large language models. By limiting adaptation to lightweight modules, it avoids interference across tasks and reduces risk of overfitting compared to full fine-tuning. The results validate {\sysname} as an efficient and performant approach to adapting pretrained models to individual tasks, without compromising on model capacity. The modular architecture enables personalized tuning on small critical parts of the model for a given task.

\noindent\textbf{Multi-task.} Prior work has shown that prompt tuning approaches deteriorate significantly when applied to multiple tasks simultaneously~\citep{wang2022multitask}. As an input-centric method similar to prompt tuning , exploring  capabilities and limits of {\sysname} in the multi-task setting is informative and can help unveil the potential of this new method.  In contrast to prompt tuning which typically sees over 10\% performance degradation in multi-task settings, AdaPrompt exhibits a minor gap of only 1-2\% versus full fine-tuning. More importantly, it achieves comparable or higher accuracy than full tuning on 6 out of 8 GLUE tasks using the FLAN checkpoint. The gap is most noticeable on the challenging CoLA task requiring complex linguistic adaptations. However, AdaPrompt's strong performance on most benchmarks shows that input-level tuning can effectively emulate task-specific behaviors.

\noindent \noindent\textbf{Analysis of rank.}

\begin{table*}[!t]
%\vspace{-0.1in}
\small

	\begin{center}
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{l|c|lc c cccccc  c c}
			\toprule \bf Setting & Checkpoint & Method& \#Tunable Param.&MNLI        &QNLI               &SST2          &QQP          &MRPC               &CoLA           &RTE        &STS-B&\bf Avg. \\ 
			                           &&&&Acc             &Acc             &Acc          &Acc            &Acc             &Mcc            &Acc            &Pearson    \\ \midrule

		    \multirow{4}{*}{\bf Single Task} & \multirow{2}{*}{FLAN} & Full Fine-tuning &11B x 8 & 92.1 & 96.0 & 97.1 & 92.2 & 92.2 & 70.1 & 93.9 & 91.2 & 90.6\\
		    &&{\sysname} & 0.008M x 8 & 91.7 & 96.1 & 97.4&90.7& 91.9& 70.0 & 94.9 & 93.0 & \textbf{90.7}\\
		    \cline{2-13} 
		   &\multirow{2}{*}{T5}&Full Fine-tuning &11B x 8 & 91.8 & 96.2 & 97.3 & 92.2 & 90.9 & 72.2 & 92.1 & 91.4  & 90.5\\
		    &&{\sysname} & 0.5M x 8  &  91.4 & 96.0 & 97.1 & 92.3 & 92.5 & 64.8 & 93.5 & 91.4 & 89.9\\
		    \midrule
		       \multirow{4}{*}{ \bf Multi-Task} & \multirow{2}{*}{FLAN} & Full Fine-tuning &11B & 91.2&96.1&97.1 & 91.9 & 90.2 & 70.2 & 93.5 & 89.5& 90.0\\
		    &&{\sysname} &0.5M &91.8 & 95.6 & 96.8 & 90.8 & 93.1 & 64.5 & 93.1 & 92.7 & 89.8 \\
		   %  &&{MOE-\sysname} &2M & \\
		     \cline{2-13} 
		   &\multirow{2}{*}{T5}&Full Fine-tuning &11B & 91.7 & 96.1 & 97.5 & 90.8 & 90.0 & 65.8 & 89.9 & 87.6 & 88.7  \\
		    &&{\sysname} &2M & 90.1 & 93.8 & 96.0 & 91.2 & 88.0 & 60.0 & 86.3 & 89.9 & 86.9\\
		   % &&{MOE-\sysname} &8M &  91.6 & 96.0 & 96.7 & 91.7 & 89.0 & 69.7 & 93.9 & 91.5 & 90.0\\

			\bottomrule
			


		\end{tabular}}
	\end{center}

	\caption{Results for NLU tasks on GLUE development set with \textbf{T5-11B}. The best result on each task is in \textbf{bold} and ``-'' denotes missing measure. Pearson refers to Pearson correlation. %Overall average performance is computed based on accuracy of QQP and MRPC.
	\#Param. denotes the number of tunable adaptation parameters used during inference.}


\end{table*}





==> subfiles/_old_pali_results.tex <==

\subsection{Multimodal Experiments}
% checkpoint details: IT
% MMIT
We conduct PEFT experiments on four VQA and two image captioning tasks using PaLI models \citep{chen2023pali}, a family of multi-modal foundational models that have achieved SoTA results on a wide range of vision and language benchmarks. We demonstrate that non-intrusive PEFT achieve very competitive results compared to full model fine-tuning for base models with higher parameter counts and instruction tuned.


\subsubsection{Base Models}
We consider four variants of PaLI models: base models at two different sizes, and whether pretraining included a multimodal instruction tuning (MMIT) stage at each size.

\textbf{PaLI models:} for the large-scale model, we consider PaLI-X \citep{chen2023pali} with 55B parameters; we use the checkpoint pre-trained per \citet{chen2023pali} with a resolution of 756 $\times$ 756.  We also consider a (relatively) small-scale model, a 5B variant of PaLI, pre-trained with similar objectives at a higher resolution (812 $\times$ 812) and better text understanding capabilities.

\textbf{MMIT:} Due to the limitation and digression of the task scopes in most public academic benchmarks, we create the MMIT task collections in the spirit of ``Self-Instruct'' \citep{wang2022self}, taking advantages of the powerful large language models. We consider 3 clusters of tasks: (i) Long-form captioning where LLMs \citep{anil2023palm} are used to combine and summarize different generated captions for each image; (ii) Creative writing where LLMs are used to generate both the novel creative writing prompts and the actual writings given the prompts based on image captions. (iii) Long-form question answering where LLMs are used to generate the both questions and answers accompanied with rationales given image captions. Although we only have 3 cluster of tasks, each cluster covers closer and comprehensive aspects to natural daily use cases. We finetune the pre-trained raw PaLI models on the MMIT collections for 17k steps to produce the MMIT checkpoints. We note the generated tasks covered in the MMIT are comprehensive yet general, we do not expect them to do directly relevant to specific down-stream tasks. In particular, we experiment on down-stream tasks that require specific skills such as understanding scene texts and documents and answering knowledge intensive questions.

\subsubsection{Implementation Details}
Fine tuning and three types of PEFT including prompt tuning \citep{prompt_tuning}, LoRA \citep{hu2021lora} and \sysname  are examined in this work. We employ adafactor \citep{shazeer2018adafactor} as the optimizer. The learning rate is set to 0.03 for the PEFT and 0.0001 for fine tuning with a linear warmup and reciprocal square root decay  if not otherwise specified. We set the dropout rate as 0.1 to prevent over-fitting. 

\textbf{LoRA.} We add LoRA weights on each linear layer in the multi-head attention and the MLP blocks in the encoder transformer blocks for all the PaLI models. Similar to \citep{yang2022prompt}, we found that adding LoRA weights in the decoder does not help the adaptation performance much at while costing twice as much as parameter counts. We use a LoRA rank of 16 in all the experiments except for the PaLI-X MMIT experiments that use a rank of 4.

\textbf{Prompt Tuning.} PT is implemented on the input to the multimodal Encoder-Decoder in PaLI, concatenating $64$ soft tunable tokens to the embeddings of the text tokens and the visual tokens from the frozen ViT. We apply two layers of residual re-parameterization \citep{razdaibiedina2023residual} for more stable results. We use a dropout rate of 0.05 for all prompt tuning experiments as we found it outperforming the default rate of 0.1

\textbf{AdaPrompt}. We insert the \sysname to the embeddings of the text tokens and the visual tokens from the frozen ViT as a non-intrusive PEFT to the PaLI's Encoder-Decoder. We use a rank of $64$ in all the experiments.



\subsubsection{Image captioning Results}

\begin{table}[h]
\scriptsize
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{1}{c|}{}         & \multicolumn{6}{c|}{PaLI-5B}                                                       & \multicolumn{6}{c}{PaLI-55B}                                                      \\ \hline
& \multicolumn{2}{c}{COCO} & \multicolumn{2}{c}{Textcaps} & \multicolumn{2}{c|}{avg. $\delta$ to FT} & \multicolumn{2}{c}{COCO} & \multicolumn{2}{c}{Textcaps} & \multicolumn{2}{c}{avg. $\delta$ to FT} \\
             & raw         & MMIT       & raw           & MMIT         & raw         & MMIT      & RAW         & MMIT       & RAW           & MMIT         & raw        & MMIT   \\\hline
FT            & 145.9       & 144.7      & 158.8         & 160.1        & 0           & 0         & 147.4       & 147        & 148.6         & 148.5        & 0          & 0        \\ 
LoRA          & 145.5       & 145.7      & 160.4         & 159.5        & +0.6        & +0.2       & 146.1       & 146.8      & 147.8         & 148.6        & -1.05      & -0.05    \\ \hline
Prompt-tuning            & 140.2       & 140.9      & 155           & 155.5        & -4.75       & -4.2      & 143.5       & 142.2      & 144.9         & 145.5        & -3.8       & -3.9     \\
\sysname      & 142.9       & 144.6      & 158.7         & 158.6        & -1.55       & -0.8      & 146.2       & 146.3      & 145.2         & 147.9        & -2.3       & -0.65    \\
\bottomrule
\end{tabular}
\caption{PEFT results on COCO and textcaps captioning tasks on the validation splits. We report cider score for each task. \sysname consistently outperforms prompt tuning as non-intrusive PEFT approaches and achieves competitive results to FT.}
\label{tab:mm_cap_results}
\end{table}

We report the PEFT image captioning cider scores \citep{vedantam2015cider} on COCO \citep{lin2014microsoft} and TextCaps \citep{sidorov2020textcaps} using the validation splits in table \ref{tab:mm_cap_results}. Within the non-intrusive PEFT family, \sysname outperforms prompt tuning by about 3 cider points on PaLI-5B and 2 cider points on the PaLI-X model, indicating the effectiveness of directly adapting the input embeddings. 

We observe smaller gaps between \sysname and FT on MMIT than the raw checkpoints for both PaLI-5B and PaLI-X models, supporting our hypothesis that PEFT approaches are able to benefit more from scaling up the pre-training tasks and demonstrate competitive results to FT. Practically speaking, as the instruction tuned LLM checkpoints occupied increasingly more market of the use case, non-intrusive PEFT, especially \sysname, become a strong candidate that significantly reduces the complexities in architecture and serving infrastructure at a cost of very minor performance degradation. As the model sizes keep growing larger and the instruction tuning tasks being more comprehensive, we expect to see even closer performance between simple non-intrusive PEFT approach like \sysname and intrusive PEFT or FT. As the non-intrusive PEFT approaches does not scale along with the depth of the growing models, they present clear advantages in terms of practicality.


\textbf{Effect of the rank.} Table \ref{tab:rank_COCO} reports the effects of changing the ranks in \sysname on COCO karparthy test set using PaLI MMIT checkpoints of both sizes. We observe that the performances are not very sensitive to the rank, indicating the stability of the \sysname. Even a rank of 4 can help the models adapt to reasonable performances and the performance saturated at a rank of 64 for the both models.


\begin{table}[h]
\centering
\begin{tabular}{l|cccc|l|cccc}
\toprule
        &  4   & 16   &  64   & 256    &        &  4  & 16   & 64   & 256   \\ \hline
PaLI-5B & 141.0   & 143.4   &  144.6   & 144.8    & PaLI-X &  144.5 & 145.3   & 146.3   & 146.3   \\ \bottomrule  
   
\end{tabular}
\caption{Effect of rank in \sysname on the COCO captioning task. }
\label{tab:rank_COCO}
\end{table}


\subsubsection{VQA Results}
In table \ref{tab:mm_vqa_results}, we present VQA performances using PEFT on four VQA tasks, covering outside knowledge VQA (OK-VQA) \citep{marino2019ok}, document understanding VQA (DocVQA) \citep{mathew2021docvqa}, and two scene-text understanding datasets, i.e. TextVQA \citep{singh2019towards} and ST-VQA \citep{biten2019scene}. We follow standard evaluation metrics, using soft accuracy \citep{antol2015vqa} for OKVQA and TextVQA and ANLS score for DocVQA and ST-VQA.


\begin{table}[h]
\scriptsize
\begin{tabular}{lc|c|cccccccccc}
\toprule
Tuning  &Non-intru- & \#params & \multicolumn{2}{c}{OKVQA} & \multicolumn{2}{c}{DocVQA} & \multicolumn{2}{c}{ST-VQA} & \multicolumn{2}{c}{TextVQA} & \multicolumn{2}{c}{avg. $\delta$ to FT}  \\
Approach   & sive &          & Raw        & MMIT         & Raw        & MMIT          & Raw          & MMIT        & Raw        & MMiT           & RAW         & MMIT            \\\midrule
FT & No & 3B$^\dag$      & 60.1       & 61.13        & 83.3       & 81.3          & 83.6         & 83.1        & 76.5       & 75.4           & 0           & 0              \\
LoRA  & No &          & 57.34      & 58.33        & 83         & 82.1          & 82.2         & 83          & 76.3       & 76.4           & -1.17       & -0.28          \\
Prompt-tuning &Yes & 131k     & 57.55      & 59.1         & 80.3       & 79.66         & 82.6         & 82.2        & 76.1       & 76.3           & -1.74      & -0.92         \\
\sysname   &Yes  & 524k     & 56.8       &  56.7    & 78.3         & 78.6      & 81.6         & 81.9        & 75.4       &   74.7     &    -2.93   & -2.33    \\\midrule
FT  & No& 32B$^\dag$       & 66.1        & 66.9        & 80.0         & 82.8        & 80.2         & 79.7        & 71.9         & 70.7         & 0.0           & 0.0       \\     
LoRA        & No& 19M    & 63.3        & 67.1        & 80.6         & 83.2        & 78.6         & 80.0        & 69.1         & 70.8         & -1.7          & +0.25         \\
Prompt tuning  &Yes& 262k     & 64.9        & 66.4        & 79.7         & 82.4        & 78.3         & 79.8        & 69.7         & 70.4         & -1.4          & -0.3           \\
\sysname     &Yes & 1.05M    & 63.9        & 66.8        &    78.3     & 82.9        & 77.9         & 80.0        &      67.8        & 70.2         &     -2.58          & -0.05          \\ \bottomrule

\end{tabular}
\caption{PEFT results on four VQA tasks on the validation splits. The first and second half present the results on the PaLI-5B and the PaLI-X models, respectively. $^\dag$ We only fine tune the Encoder-Decoder part of the PaLI model and leave the ViT part frozen. }
\label{tab:mm_vqa_results}
\end{table}


For the PaLI-5B raw model, LoRA as an intrusive PEFT approach achieves the most competitive average results to the FT results, yielding only 1.17 performance degradation where both prompt tuning and \sysname achieve worse results, yielding 1.74 and 2.93 performance degradation. We attribute this to the strong expression capabilities offered by the flexibility in modifying the internal architecture. Within non-intrusive PEFT, \sysname falls behind prompt tuning by 1.2 points. We hypothesize that the adapters in \sysname from different modalities learn to separately over fit modality bias rather than collaborating to learn to reason the visual questions given the image. 

Both issues are addressed with the help of scaling up both the parameter counts and the pre-training tasks. On the PaLI-55B MMIT model, the average performance differences on the MMIT checkpoint are negligible that only lose a score of 0.05 to FT, highlighting that \sysname emerges to be an excellent choice considering the ease of serving and the parameter counts. 

It is worth noting that all three PEFT approaches, including both intrusive and non-intrusive variants, present better performances with scaling up both parameter counts and tasks, achieving competitive performances to FT. This reveals and supports the trend towards PEFT where the LLMs and VLMs are increasingly powerful and only little adaptation is needed to achieve optimized performance for specialized use cases, relieving the need of directly learning the domain knowledge. Comparing to intrusive PEFT that are more similar to FT in spirits of adapting internal parameters, non-intrusive PEFT approaches like \sysname are often sufficient and offer similar performances with significant ease of model deployment and constant parameter counts with respect to the model depth. 
